Differential Privacy in the Shuffle Model: A Survey of Separations

Differential privacy is often studied in one of two models. In the central model, a single analyzer has the responsibility of performing a privacy-preserving computation on data. But in the local model, each data owner ensures their own privacy. Although it removes the need to trust the analyzer, local privacy comes at a price: a locally private protocol is less accurate than a centrally private counterpart when solving many learning and estimation problems. Protocols in the shuffle model are designed to attain the best of both worlds: recent work has shown high accuracy is possible with only a mild trust assumption. This survey paper gives an overview of novel shuffle protocols, along with lower bounds that establish the limits of the new model. We also summarize work that show the promise of interactivity in the shuffle model.

==> amplification.tex <==
\section{Amplification: Building Shuffle Protocols from Local Protocols}
In the setting where each user $i$ has a bit $x_i\in \zo$, the canonical local protocol is \emph{randomized response} which we shorthand $\rr$.\anote{Warner} In this protocol, user $i$ reports a bit drawn from $\Ber(1/2)$ with probability $p$ and otherwise report $x_i$. Setting $p=\frac{2}{e^\eps+1}$ suffices for $\eps$-local privacy.

If we shuffle all $n$ messages of $\rr$, we would have a one-message shuffle protocol. Intuitively, the fact that an adversary has to sift through many noisy bits makes it much more difficult to determine the actual data of a target user. This means we can obtain a shuffle protocol with some target privacy level by choosing a local protocol\footnote{Some protocols will have to be modified to apply this technique. For example, a local protocol may partition public coins amongst users but shuffling their messages together breaks the linkage between users and coins.} with weaker privacy (e.g. smaller noise probability $p$ in $\rr$).

\emph{Amplification lemmas} quantify the intuition. One is due to Erlingsson et al. \cite{EFMRTT19}.
\begin{lem}
If $\cR$ is an $\eps$-locally private randomizer where $\eps < 1/2$, then for any $n>1000$ and $\delta<1/100$, $(\cS\circ\cR^n)$ is $\left( \eps',\delta \right)$-shuffle private where $\eps' = 12\eps \cdot \sqrt{\frac{\log (1/\delta)}{n}}$.
\end{lem}
This statement is obtained by a careful use of amplification by subsampling and advanced composition. We remark that the technique also applies to the case where \emph{users} are shuffled (instead of messages), so that the amplification lemma holds even for interactive local protocols.

Balle et al \cite{BBGN19} give an amplification lemma that holds for a broader range of $\eps$.
\begin{lem}
If $\cR$ is an $\eps$-locally private randomizer, then for any $n$ and $\delta$ such that $e^\eps < \sqrt{\frac{n}{\log (1/\delta)}}$, $(\cS\circ\cR^n)$ is $\left( \eps',\delta \right)$-shuffle private where $\eps' = O\left( \min(\eps,1)\cdot e^\eps\cdot \sqrt{\frac{\log (1/\delta)}{n}} \right)$.
\end{lem}
To prove this theorem \cite{BBGN19} first show that the randomizer is the mixture of a data-dependent distribution and a data-independent \emph{blanket} noise distribution. Formally, $\cR(x) = (1-p)\cdot \hat{\cR}(x) + p\cdot \bD_\cR$. In the case of $\rr$, the blanket is simply $\Ber(1/2)$. By concentration of the binomial distribution, there are $\Theta(pn)$ samples from the blanket $\bD_\cR$. Then they argue that shuffling a sample from $\hat{\cR}(x)$ with $\Theta(pn)$ blanket samples is an $(\eps',\delta)$ differentially private algorithm. This is managed by tracking how each additional blanket sample affects the hockey-stick divergence, a quantity which directly corresponds to approximate differential privacy.

\begin{rem}
This method of constructing shuffle protocols immediately implies robust shuffle privacy: if only a $\gamma$ fraction of users obey the protocol, then the analysis simply changes from using $n$ in the amplification lemma to $\gamma n$.
\end{rem}
